Parameter-Efficient Sparse Retrievers and Rerankers using Adapters

Parameter-Efficient transfer learning with Adapters have been studied in Natural Language Processing (NLP) as an alternative to full fine-tuning. Adapters are memory-efficient and scale well with downstream tasks by training small bottle-neck layers added between transformer layers while keeping the large pretrained language model (PLMs) frozen. In spite of showing promising results in NLP, these methods are under-explored in Information Retrieval. While previous studies have only experimented with dense retriever or in a cross lingual retrieval scenario, in this paper we aim to complete the picture on the use of adapters in IR. First, we study adapters for SPLADE, a sparse retriever, for which adapters not only retain the efficiency and effectiveness otherwise achieved by finetuning, but are memory-efficient and orders of magnitude lighter to train. We observe that Adapters-SPLADE not only optimizes just 2\% of training parameters, but outperforms fully fine-tuned counterpart and existing parameter-efficient dense IR models on IR benchmark datasets. Secondly, we address domain adaptation of neural retrieval thanks to adapters on cross-domain BEIR datasets and TripClick. Finally, we also consider knowledge sharing between rerankers and first stage rankers. Overall, our study complete the examination of adapters for neural IR

==> old_msmarco.tex <==
\begin{table}
\caption{Evalutation on MS MARCO dev set, TREC DL 2019 and TREC DL 2020}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cc|cc|cc|c|c}
\hline
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Pretrained Model}} & \multicolumn{2}{c|}{\textbf{MS MARCO dev}} & \multicolumn{2}{c|}{\textbf{TREC DL 2019}} & \multicolumn{2}{c|}{\textbf{TREC DL 2020}} & \multirow{2}{*}{\textbf{Flops}} & \multirow{2}{*}{\textbf{\makecell{Training \\ Params}}} \\
& &  MRR@10 & R@1000 & NDCG@10 & R@1000 & NDCG@10 & R@1000 & & \\
\hline
%SPLADE-$l_{Flops}$ &  & 0.322 & 0.955 & 0.665 & 0.813 & & & 0.73 \\
%SPLADE-$l_1$ & & 0.322 & 0.954 & 0.667 & 0.792 & & & 0.88 \\
%SPLADE$_{max}^1$ & distilbert & 0.340 & 0.965 & 0.684 & 0.851 & & & 0.73 & 66362880 \\
\multirow{3}{*}{SPLADE$_{max}^1$} & distilbert & 0.346 & 0.963 & 0.691 & 0.80 & 0.677 & 0.85 & 1.43 & 100\% \\
& cocondenser & 0.359 & 0.971 & 0.689 & 0.807 & 0.680 & 0.842 & 1.21 & 100\% \\
& cocondenser-MLM & 0.366 & 0.977 & 0.712 & 0.814 & 0.684 & 0.853 & 1.09 & 100\% \\

\hline
\textbf{Mono} & distilbert & 0.351 & 0.968 & 0.711 &  0.839 & 0.676 & 0.778 & 1.44 & 2.23\% \\
\textbf{Adapters-} & cocondenser & 0.361 & 0.977 & 0.695 & 0.845 & 0.688 & 0.782 & 1.97 \\
\textbf{SPLADE}$^1$  & cocondenser-MLM & 0.376 & 0.980 & 0.712 & 0.839 & 0.688 & 0.785 & 0.80 &  \\
 \hline
 \hline
 \multirow{3}{*}{SPLADE$_{distil}^1$} & distilbert & 0.371 & 0.979 & 0.727 & 0.866 & 0.711 & 0.892 & 3.93 &  \\
 & cocondenser & 0.386 & 0.984 & 0.735 & 0.868 & 0.730 & 0.899 & 4.28 & \\
  & cocondenser-MLM & 0.388 & 0.982 & 0.734 & 0.865 & 0.732 & 0.901 & 4.38 & \\
 \hline
\textbf{Adapters-} & distilbert & 0.361 & 0.972 & 0.711 & 0.847 & 0.693 & 0.818 & 1.86 & \\
\textbf{SPLADE-} & cocondenser & 0.384 & 0.980 & 0.724 & 0.860 & 0.719 & 0.827 & 2.23 & \\
\textbf{distil}$^1$ & cocondenser-MLM & 0.390 & 0.983 &  0.740 & 0.869 & 0.730 & 0.835 & 2.34 & \\
\hline
\hline
\textbf{Bi} & distilbert & 0.352 & 0.967 & 0.690 & 0.813 & 0.666 & 0.774 & 0.74 &  \\
\textbf{Adapters-} & cocondenser & 0.365 & 0.976 & 0.710 & 0.828 & 0.686 & 0.787 & 1.01 & 2.16\% \\
\textbf{SPLADE}$^2$  & cocondenser-MLM & 0.372 & 0.976 & 0.701 & 0.839 & 0.700 & 0.783 & 0.37 & 2.16\%\\
\end{tabular}
}
\label{tab:spalde_adapters_results}
\end{table}
